It Takes Two to Tango: Serverless Workflow Serving via Bilaterally Engaged Resource Adaptation

Serverless platforms typically adopt an early-binding approach for function sizing, requiring developers to specify an immutable size for each function within a workflow beforehand. Accounting for potential runtime variability, developers must size functions for worst-case scenarios to ensure service-level objectives (SLOs), resulting in significant resource inefficiency. To address this issue, we propose Janus, a novel resource adaptation framework for serverless platforms. Janus employs a late-binding approach, allowing function sizes to be dynamically adapted based on runtime conditions. The main challenge lies in the information barrier between the developer and the provider: developers lack access to runtime information, while providers lack domain knowledge about the workflow. To bridge this gap, Janus allows developers to provide hints containing rules and options for resource adaptation. Providers then follow these hints to dynamically adjust resource allocation at runtime based on real-time function execution information, ensuring compliance with SLOs. We implement Janus and conduct extensive experiments with real-world serverless workflows. Our results demonstrate that Janus enhances resource efficiency by up to 34.7% compared to the state-of-the-art.

==> section/04-profiler.tex <==
\section{Profiler}
\label{sec:profilier}
Here,  we discuss how to profile function execution latency.
Based on that, two metrics are proposed as a preparation for synthesizing hints.
\subsection{Diverse percentiles based profiling}
As explained in \S{\ref{sec:bg:worst-case}}, function execution latency is a distribution, making the current work, which either depends on a single statistic or a simple 99\% percentile distribution, insufficient.
To fix this issue, for any given batch sizes we introduce diverse percentile latency distributions to profile the execution latency, which is expressed as $L(p,k)$, with CPU cores and percentiles denoted as $k$ and $p$, respectively.

\subsection{Timeout and resilience.}
The diversity in percentiles enables more opportunities to explore higher resource efficiency but comes at the risk of SLO violations.
Specifically, when setting percentiles lower than 99\%, it may incur under-estimation of function execution, making functions prone to \textit{timeout}, i.e., their actual execution latency over the estimated latency.
Timeout is expressed as follows
\begin{eqnarray}
     D(p,k) = L(P_{99},k) -L(p,k).
\end{eqnarray}

Consequently, for preventing from SLO violation, \namex has to provision more CPU cores to downstream functions to absorb previous timeout.
Moreover, we propose another metric called \emph{resilience} to quantify the absorption capability, which is expressed as follows
\begin{eqnarray}
    R(p,k)= L(p,K_M)-L(p,k),
\end{eqnarray}
where $k_M$ denotes the maximum available CPU cores.
Notably, timeout must be restricted within the upper bound of resilience, such that SLO can be guaranteed.

 









==> section/06-adapter.tex <==
\section{Adapter}
\label{sec:adapter}
\begin{algorithm}[!t]
    
	\caption{Adapt resource online \jing{(necessary?)}}
 	\LinesNumbered    
    \KwIn{$\mathbf{F}= \left\langle f_1,\dots,f_N \right\rangle$: (sub-)workflow}
    \KwIn{$\mathbf{U}, T$: hints table and time budget/slack}
    \KwOut{$k$: CPU cores for head function}
	\SetKwFunction{FMain}{\texttt{adapt}}
    \SetKwProg{Fn}{Function}{:}{}
    
    \Fn{\FMain{$\mathbf{F},\mathbf{U}, T$}}{
    $ i \leftarrow \mathbf{U}.$\texttt{index}($T$)\\
    \If{$i=\emptyset$}
    {
    $\mathbf{K} \leftarrow $\texttt{generate}($\mathbf{F},T, \emptyset$) \\
    $\mathbf{U} \leftarrow $\texttt{condense}($\{\left \langle T, \mathbf{K}\right\rangle\}$)\\
    }
    \Else{
    $\mathbf{K} \leftarrow \mathbf{U}[i]$
    }
    \text{return}~$\mathbf{K}[0]$
    }
\label{alg:adapt}
\end{algorithm}

Having demonstrated how to offline synthesize and condense hints, we now focus on utilizing the hints table to accomplish online adaptation.

As outlined in \S~\ref{sec:system-overview},  after each function's execution, adapter re-evaluates the available time budget for the remaining functions while adapting the head function's size accordingly.
The procedure of adapter is listed in Algorithm~\ref{alg:adapt}.
Specifically, it first accesses the sub-workflow's hints table $\mathbf{U}$ to figure out the proper hint that can well meet the required time budget $T$ with the minimum resource consumption (Line 2).
Notably, if the above searching suffers a miss hit, due to the dynamics at runtime (detailed in~\S~\ref{sec:bg:worst-case}), adapter will revoke synthesizer to generate the proper hint on spot while updating it into the table (Line 3--5).
Moreover, adapter continuously counts the above miss. 
When it exceeds a predefined threshold, adapter argues that execution latency distribution may change, when adapter will trigger a holistic update of both profiler and synthesizer, for maintaining adaptation's accuracy.

\begin{algorithm}[!t]
    \caption{Adapt resource online \label{alg:janus:adapt}}
    \LinesNumbered    
    \KwIn{$\mathbf{F}= \left\langle f_1,\dots,f_N \right\rangle$: (sub-)workflow}
    \KwIn{$\mathbf{U}, T$: hints table and time budget/slack}
    \KwOut{$k$: CPU cores for head function}
	\SetKwFunction{FMain}{\texttt{adapt}}
    \SetKwProg{Fn}{Function}{:}{}
    
    \Fn{\FMain{$\mathbf{F},\mathbf{U}, T$}}{
    $ i \leftarrow \mathbf{U}.$\texttt{index}($T$)\\
    \If{$i=\emptyset$}
    {
    $\mathbf{K} \leftarrow $\texttt{generate}($\mathbf{F},T, \emptyset$) \\
    $\mathbf{U} \leftarrow $\texttt{condense}($\{\left \langle T, \mathbf{K}\right\rangle\}$)\\
    }
    \Else{
    $\mathbf{K} \leftarrow \mathbf{U}[i]$
    }
    \text{return}~$\mathbf{K}[0]$
    }

\end{algorithm}

==> section/09-discuss.tex <==
\section{Discussion}
\label{sec:discuss}
\jing{Janus maintains a warm pod pool to decrease the impact of cold start.
Despite its simplicity, this pool may inevitably compromise resource efficiency.
Additionally, Janus may exhibit sub-optimal resource adaptation for dynamic workflows with uncertain execution paths.
This uncertainty exacerbates the dependencies of adaptation decisions (as detailed in \S\ref{sec:bg:adaptive-allocation}), potentially leading to sub-optimal adaptation especially for functions shared across different paths.}








==> section/backup.tex <==
\section{Related-work}
Optium~\cite{eurosys23-optium} conducts data-driven analysis of Alibaba unified scheduler, which further confirms the predictability of applications' running performance.

\subsection{Performance interference}
\begin{itemize}
    \item ProPack~\cite{hpdc23-propack}.This work unlocks the potential of serverless computing to support high-parallel applications.Yet, the empirical study reveals that current platforms fail to establish the required number of concurrent function instances simultaneously, resulting in substantial scaling time, i.e., the time between the start of the first function instance and the start of the last instance. ProPack proposes to pack multiple functions into one function instance to lower the scaling time. Particularly, Propack notices the performance interference among co-located functions while formulating the interference concerning function types and the degree of packing degree (i.e., the optimal number of functions packed together). This work however overlooks a thorough analysis of the root cause of performance interference.
    \item Long-term profiling~\cite{sesame23-night-shift}. Schirmer et al. conducted a long-term study of serverless systems in three aspects: request-response latency, unexpected cold starts, and long-term trends.Specifically, this work evaluated three functions, including floating point operations, matrix function, and face detection, which are invoked every 40 seconds over multiple months.
    The results suggest that \textit{latency of up to 15\% and more than three times as many unexpected cold starts from day to night within the same day, and these effects are most noticeable at the start of the week.}
    \item X86 vs ARM~\cite{icpe22-x86-vs-arm}. This work reveals the impacts of CPU types, i.e., X86 and ARM on function performance. Meanwhile, it illustrates the correlation between CPU steal time and performance degradation.
    \item Serverless isn't server-less~\cite{wosc20-serverless-not-server-less}.
    The contention for shared resources, such as CPU, CPU cache, network, and IO, in serverless computing is fully explored. 
    Depending on AWS Lambda, the results show that compared with CPU-bound functions, network function suffers severe performance variation.
    \item CPU-TAMS~\cite{ic2e22-cpu-tams}.
    CPU-TAMS fully explores the resource-to-memory mappings, i.e., the number of allocated resources like vCPU cores and network/IO throughput given specific memory sizes of,  of different serverless platforms.
    Based on the empirical analysis, this work proposed a function size recommendation strategy based on CPU times.
    \item ServerlessBench\cite{socc20-serverlessbench}. This benchmarks demonstrates the performance of different serverless platforms in the aspects of communication latency, starup latency, stateless execution, and  resource effciency as well as performance isolation.
    Notably, it validates the inefficient isolation for memory bandwidth and CPU cores among co-located functions in commercial platforms (Ant Financial).
    \item Huawei cloud~\cite{socc23-huawei-cloud}. This production trace reveals the features of workloads in Huawei cloud while quantifying delays of functions throughout their holistic life cycle.
    \item SeBS~\cite{middleware21-sebs}. SeBS reports the wide latency distributions of I/O bound (network and disk) functions.
\end{itemize}


\subsection{Early-bind}

\jing{Aquatope~\cite{asplos23-aquatope} and FIRM~\cite{osdi20-firm} take into account runtime performance interference (uncertainty) to decide function sizes.}

\jing{ORION~\cite{osdi22-orion} and WISEFUSE~\cite{mac22-wisefuse} observe high variability and the skew in function execution latency and develop a distribution-based performance modeling to provision serverless DAGs.}


COSE~\cite{infocom20-cose} utilizes statistical Learning to learn the cost/performance of functions with respect to different sizes.
Then, it selects the ``best" size for a single function or a chain of function to minimize the overall costs without violating SLOs.



FA2~\cite{rtas22-fa2} fully considers the dependency of functions within a workflow as well as their uncertain execution paths to periodically adapt resources to minimize resource consumption while promising SLAs.


SIMPPO~\cite{socc22-simppo} utilizes online learning to boost resource management in serverless.

Parrotfish~\cite{socc23-parrotfish} employs online parametric regression to learn the relationship between function execution latency and memory sizes, and find the most cost-optimal sizes for a single function, with latency constraints.

%rely on elastic batching to achieve higher inference throughput for serverless deep learning workloads, without violating SLOs. 



Cypress~\cite{socc22-cypress} enables input size-aware request batching and resource provisioning for input size-sensitive applications (e.g., sentiment analysis). 
Atoll~\cite{socc21-atoll} enables proactive resource scaling as well as deadline-aware scheduling to minimize SLO violations.

Fifer~\cite{middleware20-fifer} leverages the slacks, generated at each stage, to adjust batch sizes and scale out/in containers for higher resource utilization with SLO guarantees.

Erms~\cite{asplos23-erms} systematically evaluate latency targets for shared microservices while adjusting their sizes to minimize resource consumption.

ReSC~\cite{arxiv22-resc} and FUSIONIZE~\cite{ic2e22-fusionize} propose newly resource-centric, distinct from current function-centric, serverless architecture for striking the trade-off between flexibility and performance.





On the other hand, there exists research from both the industry and the academic that concentrate on selecting the optimal function sizes for developers, such as AWS Lambda Power Turing~\cite{lambda-tuning}, AWS Compute Optimizer~\cite{lambda-compute-optimizer}, Sizeless~\cite{middleware21-sizeless} and COSE~\cite{infocom20-cose}.



\subsection{Late-bind}

Nevertheless, current offline hints hold compromised accuracy~\cite{middleware21-sizeless,infocom20-cose,socc23-parrotfish,socc22-cypress}, due to their simplistic modeling of execution latency or ad-hoc threshold-based rules; meanwhile, online hints suffer unsatisfactory time-efficiency owing to their complex formulations, e.g., transform resource adaptation into optimization problems ~\cite{rtas22-fa2,infocom22-stepconf,icdcs23-joint-video-analyze}.

\jing{BATCH~\cite{sc20-batch} fully considers serverless workload burstiness (the intensity of arrival requests) to dynamically adjust function size (memory size) and batching parameters, for the sake of minimizing monetary cost without violating SLOs.}

\jing{Kraken~\cite{socc21-kraken} and Xanadu~\cite{middleware20-xanadu} employ proactive and reactive resource scalers simultaneously to provision dynamic DAG workloads, which have uncertain execution paths, aiming to minimize resource consumption without SLOs violations.}

\textbf{Morhpling~\cite{socc21-morphling}, Llama~\cite{socc21-llama}, and INFaaS~\cite{socc21-llama} focus on resource auto-configuration.}

Llama


\jing{Apart from auto-scaling, there are work focusing on serverless workflows scheduling,  i.e., when, where, and how to run functions. 
For example, Sequoia~\cite{socc20-sequoia} offers multiple scheduling policies available to providers/developers to alleviate issues mid-chain drops.}

\section{Exp}
\mypara{Workflows}
Setups for motivation. We implement four different types of functions as follows:
\begin{itemize}
    \item \textbf{CPU-intensive}. AES encryption for a text with size as 100KB~\cite{isca22-lukewarm}.
    \item \textbf{Memory-intensive}. Read data, with the size as 50MB and 100MB, from a locally deployed Redis.
    \item \textbf{Network-intensive}. Send data, with the size as 1MB and 5MB, to a remote server through network sockets.
    \item \textbf{IO-intensive}. Use os.fsync to write data, with the size as 1MB and 5MB, to the local disk~\cite{atc18-peek-bench}.
\end{itemize}

We configure all the above functions with the same size as one CPU core and memory with 500MB while fixing their concurrency as one, i.e., each instance can only process one request at once.
Additionally, the VM, which deploys the function instances, occupies eight CPU cores and 10752MB while limiting the maximum scale of instances to six.

==> section/extend.tex <==
\begin{document}
1. scenarios: dynamic DAG, which impacts the synthesizing of hints
2. optimization objectives: minimize the impacts of cold start
\end{document}

==> section/to-do-list.tex <==
% \mypara{design}
% \begin{itemize}
%     \item dynamic DAGs:
%     \item cold start
%     %当前只针对链式workflow的adaptive allocation，未来将支持更复杂的，比如具有分支、并行结构的workflow；2）系统未能充分利用最后一个函数的slack，影响最终的优化效果；3）adaptation会放大冷启动的影响，未来需要引入execution variability-aware的保活、预热机制。
% \end{itemize}

% \mypara{exps}
% \begin{itemize}
%     \item impacts of miss threshold
%     \item impact of $C$ when synthesizing hints
%     \item impact of percentile ranges  when synthesizing hints
% \end{itemize}

% \mypara{implementation}
% \begin{itemize}
%     \item how to implement synthesizer and profiler
%     \item how the adpater interact with the other components
%     \item how the adapter interact with the platforms=> resource adapatation decision is rewriten into a yaml.
%     %1. 如何高效实现面向k8s的resource adaptation；
%     %2. 如何实现adapter，能让其和现有平台高效交互
% \end{itemize} 


